About the Complexity of Two-Stage Stochastic IPs

We consider so called $2$-stage stochastic integer programs (IPs) and their generalized form of multi-stage stochastic IPs. A $2$-stage stochastic IP is an integer program of the form $\max \{ c^T x \mid Ax = b, l \leq x \leq u, x \in \mathbb{Z}^{nt + s} \}$ where the constraint matrix $A \in \mathbb{Z}^{r \times s}$ consists roughly of $n$ repetition of a block matrix $A$ on the vertical line and $n$ repetitions of a matrix $B \in \mathbb{Z}^{r \times t}$ on the diagonal. In this paper we improve upon an algorithmic result by Hemmecke and Schultz form 2003 to solve $2$-stage stochastic IPs. The algorithm is based on the Graver augmentation framework where our main contribution is to give an explicit doubly exponential bound on the size of the augmenting steps. The previous bound for the size of the augmenting steps relied on non-constructive finiteness arguments from commutative algebra and therefore only an implicit bound was known that depends on parameters $r,s,t$ and $\Delta$, where $\Delta$ is the largest entry of the constraint matrix. Our new improved bound however is obtained by a novel theorem which argues about the intersection of paths in a vector space. As a result of our new bound we obtain an algorithm to solve $2$-stage stochastic IPs in time $poly(n,t) \cdot f(r,s,\Delta)$, where $f$ is a doubly exponential function. To complement our result, we also prove a doubly exponential lower bound for the size of the augmenting steps.

==> schrott.tex <==
y applying the above lemma recursively, we obtain the following lemma for the intersection of several integer cones.
\begin{lemma}\label{lem:intersection_all}
    Given integer cones $int.cone(B^1), \ldots , int.cone(B^\ell)$ for base matrices $B^1, \ldots , B^\ell \subset \ZZ^{d}$ with $\norinf{B^i} \leq \Delta$ and consider the integer cone of the intersection $int.cone(\hat{B}) = \bigcap_{i=1}^\ell int.cone(B^i)$ for some generating set of elements $\hat{B}$.
    
    Then for each indecomposable element $b \in int.cone(\hat{B})$ with $B^i \lambda^i = b$ for some $\lambda^i \in \ZZ^{B^i}$ in the intersection cone, we have that $\norone{\lambda^i} \leq \Delta^{O(d^{\lceil \log(\ell) \rceil + 1})}$ for all $1 \leq i \leq \ell$.
\end{lemma}
\begin{proof}
    Given $int.cone(B^1), \ldots , int.cone(B^\ell)$, we can apply Lemma \ref{lem:intersectiontwo}, to two consecutive integer cones each and obtain the set of pairwise intersected integer cones
    \begin{align*}
        int.cone(\BB^{1}[1]) &= int.cone(B^1) \cap int.cone(B^2) \\ int.cone(\BB^{2}[1]) &= int.cone(B^3) \cap int.cone(B^4)\\
        & \vdots
    \end{align*} 
    for some generating sets $\BB^1[1], \ldots , \BB^{\lceil \ell/2 \rceil}[1] \subset \ZZ^d$.
    In the next iteration, we can apply the same procedure to build the pairwise intersection of the inter cones generated by $\BB^1[1], \ldots, \BB^{\lceil \ell/2\rceil}[1]$ and we can repeat this procedure inductively until we obtain a single integer cone $int.cone(\hat{B})$ with $int.cone(\hat{B}) = \bigcap_{i=1}^\ell int.cone(B^i)$.
    We call the respective generating sets of the $t$-th iterations $\BB^j[t]$ for $j = 1 , \ldots , \lceil \frac{\ell}{2^t} \rceil$. Hence, we obtain
    \begin{align*}
        int.cone(\BB^1[t+1]) &= int.cone(\BB^1[t]) \cap int.cone(\BB^2[t])\\ int.cone(\BB^{2}[t +1]) &= int.cone(\BB^{3}[t]) \cap int.cone(\BB^{4}[t]).\\
        \vdots
    \end{align*}
    In the following we show by induction that $\norinf{b} \leq (3 d \Delta)^{(d+2)^t}$ for any $b \in \BB^j[t]$ and any set of generating elements $\BB^j[t]$ in the $t$-th iteration. Clearly it is true for $t=0$ as $\norinf{b} \leq \Delta$ for $b \in \BB^i$.
    %$b$ can be written by $b = B^ \lambda$ for any $\lambda^j$ with $\norone{\lambda^j} \leq $ and that for every and that $\norinf{b} \leq (3 d \Delta)^{(d+2)^t}$.
    
    Now consider a $b \in \BB^j[t+1]$ for some $j$.
    According to Lemma \ref{lem:intersectiontwo}, we have for each generating element $b \in \BB^j[t+1]$ that there exists for the corresponding generating sets $\BB^i[t]$ of the previous iterations a $\lambda \in \ZZgeq^{B^i[t]}$ with $B^i[t] \lambda = b$ such that $\norone{\lambda} \leq (2d \Delta' +1)^d \leq (3d \Delta)^d$, where $\Delta'$ is the size of generating elements in $\BB^j[t]$. By induction hypothesis $\Delta' \leq \Delta (3d \Delta)^{(d+2)^{t}}$.
\begin{align*}
    \norone{\lambda} \leq (3d(3d \Delta)^{(d+2)^{t}})^d = (3d)^d (3d \Delta)^{(d+2)^{t}d} < (3d \Delta)^{d(d+2)^{t}+d}
\end{align*}
\begin{align*}
    \norinf{b} & \leq \Delta' \cdot \norone{\lambda} \leq (3d \Delta)^{d(d+2)^{t}+d} (3 d \Delta)^{(d+2)^t} = (3d \Delta)^{d(d+2)^{t}+d + (d+2)^t} \\ & < (3 d \Delta)^{(d+2)(d+2)^{t}} = (3 d \Delta)^{(d+2)^{t+1}}
\end{align*}
    
    It remains to prove that for any $b \in \hat{\BB}$ there exists a vector $\lambda \in \ZZgeq^{\BB^i}$ for each $i = 1, \ldots , \ell$ with $\BB^i \lambda = b$ such that $\norone{\lambda} \leq $. 
    Again, we will prove this by induction. Therefore, let $b \in \BB^j [t+1]$.
    As shown above, $b$ can be represented by elements of the corresponding set $\BB^i[t]$ of the previous iteration i.e. $b = \sum_{x \in \BB^i[t]} \lambda_x x$ for some $\lambda \in \ZZgeq^{\BB^i[t]}$ with $\norone{\lambda} \leq (3d \Delta)^{d(d+2)^{t}+d} \leq (3 d \Delta)^{(d+2)^{t+1}}$.
    Furthermore, each $x \in \BB^i[t]$ can be represented by $x = \BB^i \gamma^x$ and hence
    \begin{align*}
        b = \sum_{x \in \BB^i[t]} \lambda_x x = \sum_{x \in \BB^i[t]} \lambda_x (\BB^{i} \gamma^x) = \sum_{x \in \BB^i[t]} \BB^{i} (\lambda_x \gamma^x) .
    \end{align*}
    By induction hypothesis we know that $\norone{\gamma^x} \leq (3d\Delta)^{(d+2)^{t}}$ for every $x \in \BB^i[t]$.
    
    %Hence, $b \in \BB^j [t+1]$ can finally be represented by elements of $b = \BB^i (\gamm)$ and their size is bounded by 
    %\begin{align*}
    %   b = \sum_{j=1}^{|\CC^{\lceil i/ 2 \rceil}|} \CC^{\lceil i/ 2 \rceil}_j \gamma_j = \sum_{j}^{|\CC^{\lceil i/ 2 \rceil}|} B^{i} \lambda^j \gamma_j
    %\end{align*} where $B^i \lambda^j = \CC^{\lceil i/ 2 \rceil}_j$. 
    The size of the components can hence be bounded by
    \begin{align*}
        \norone{ \sum_{x \in \BB^i[t]}(\lambda_x \gamma^x) } 
        \leq \sum_{x \in \BB^i[t]} \norone{\lambda_x \gamma^x} =  \sum_{x \in \BB^i[t]} \lambda_x \norone{\gamma^x} 
        \leq (3d\Delta)^{(d+2)^{t}} \sum_{x \in \BB^i[t]} \lambda_x \\
        \leq (3d\Delta)^{(d+2)^{t}} (3 d \Delta)^{(d+2)^{t+1}}
        \leq (3d\Delta)^{(d+2)^{t+2}}
    \end{align*} 
    Hence we obtain that each generating element $b$ of an integer cone in the $t$-th iteration can be written by $b = B^i \lambda$ for some $\lambda \in \ZZgeq^{B^i}$ with $\norone{\lambda} \leq (3d\Delta)^{(d+2)^{t+1}}$. Since we need $\lceil \log (\ell) \rceil$ iterations to obtain $int.cone(\hat{B})$, we get the desired bound of $\Delta^{O(d^{\lceil \log(\ell) + 1 \rceil})}$.
\end{proof}



In this paper the authors consider classical linear integer programming, where the objective is to find a vector x >=0 that satisfies a system of equalities Ax = b for a matrix A and a right hand side vector b. They present new lower bounds on the running time for the problem of finding a feasible solution for a given integer program.

Recently there has been significant progress in the area of integer programming and new algorithms have been developed with a running time of the form (m ||A||_\infty)^O(m) log ||b||, where m is the number of rows of the matrix.
The authors main contribution is to show that for {0,1}-matrices the m log m term in the exponent is tight under the exponential time hypothesis. Similar lower bounds have been known before, but it was unclear if the log term in the exponent is actually needed.
To show the lower bound, the authors use an interesting technique of so called detecting matrices. The techniques are based around the idea that n objects with each having a possible weight of {1, ... , d} can be determined by weighing only m/(log_d m) subsets of the given items (instead of the trivial approach of using m weightings, where every single item is weighed once).

Furthermore, the authors show a double exponential lower bound dependency for the structural parameter of an IP which is called the dual treedepth. For this the authors use techniques to reduce the coefficients of the IP by increasing its treedepth.

In general the paper does not bring a major new technical innovations. But it brings an interesting new technique to a highly relevant area. Therefore I think that the paper can be accepted.




\begin{theorem}
    Let $y$ be an indecomposable cycle of matrix $\mathcal{M}$ then $\norinf{y}$ is bounded by a function $T(s_1, \ldots , s_{t},r)$, where $t$ is the depth of the tree. The functions $T$ involves a tower of $t$ exponentials.
\end{theorem}
\begin{proof}
Consider a submatrix $\mathcal{A}$ of the constraint matirx $\mathcal{M}$ corresponding to a subtree of the tree with depth $t$. Hence, $\mathcal{A}$ itself is of multi-stage stochastic structure. Let submatrix $A \in \{A^{(1)}, \ldots , A^{(\ell)} \}$ be the root of the corresponding subtree of $\mathcal{A}$ and let the submatrices $B^{(1)}, \ldots , B^{(n)}$ be the submatrices corresponding to the subtrees of $A$ with $rows(B^{(i)}) \subseteq rows(A)$ for all $1 \leq i \leq n$.

Let $\bar{A}^{(i)}$ be the submatrix of $A$ which consists only of the rows that are used by $B^{(i)}$ (recall that $rows(B^{(i)}) \subseteq rows(A)$). Now suppose that $y$ is a cycle of $\mathcal{A}$, i.e. $\mathcal{A} y =0$ and let $y^{(0)}$ be the subvector of $y$ consisting only of the entries that belong to matrix $A$. Symmetrically let $y^{(i)}$ be the entries of vector $y$ that belong only to the matrix $B^{(i)}$ for $i>0$.  
Since $\mathcal{A}y = 0$ we also know that $\bar{A}^{(i)}y^{(0)} + B^{(i)}y^{(i)} = (\bar{A}^{(i)} B^{(i)}) \begin{pmatrix} y^{(0)} \\ y^{(i)} \end{pmatrix}= 0$ for every $1 \leq i \leq n$. 
Each vector $\begin{pmatrix} y^{(0)} \\ y^{(i)} \end{pmatrix}$ can be decomposed into a set of indecomposable cylces $C_i$ , i.e. 
\begin{align*} \begin{pmatrix} y^{(0)} \\ y^{(i)} \end{pmatrix}
   = \sum_{c \in C_i} c
%   =  \begin{pmatrix} z^{(i_1)} \\ \bar{z}^{(i_1)} \end{pmatrix} + \ldots
%   + \begin{pmatrix} z^{(i_{\ell_i})} \\ \bar{z}^{(i_{\ell_i})} \end{pmatrix},
\end{align*}
where each cycle $c \in C_i$ is a vector $c = \begin{pmatrix} c^{(0)} \\ c^{(i)} \end{pmatrix}$ consisting of subvector $c^{(0)}$ of entries that belong to matrix $A$ and a subvector $c^{(i)}$ of entries that belong to the matrix $B^{(i)}$.
Note that the matrix $(A^{(i)} B^{(i)})$ has a multi-stage stochastic structure with a corresponding tree of depth $t-1$.
Hence, by induction we can assume that each indecomposable cycle $c \in C_i$ is bounded by $\norinf{c} \leq T(s_1, \ldots , s_{t-1}, r)$ for all $1 \leq i \leq n$, where $T$ is a function that involves a tower of $t-1$ exponentials.
In the base case that $t=0$ and the matrix $\mathcal{A}$ only consists of one block matrix, we can bound $\norinf{c}$ by $(2 \Delta+1)^r$ using Theorem \ref{thm:Graver_bound}.
Let $p$, be the projection that maps a cycle to the entries that belong the matrix $A$ i.e. $p(c) = p(\begin{pmatrix} c^{(0)} \\ c^{(i)} \end{pmatrix}) = c^{(0)}$.

For each vector $\begin{pmatrix} y^{(0)} \\ y^{(i)} \end{pmatrix}$ and its decomposition into cycles $C_i$ let $p(C_i) = \{ p(c) \mid c \in C_i \}$. Since
\begin{align*}
    y^{(0)} = \sum_{c \in C_1} p(c) = \ldots = \sum_{c \in C_n} p(c)
\end{align*}
we can apply Lemma \ref{lem:subrepresentation}, to obtain subsets $S_i \subseteq p(C_i)$ of bounded size \begin{align*}
    |S_i| \leq (s_t T)^{O(s_t (T^{s_{t}^2}))} = 2^{T^{O(s_{t}^2)}}
\end{align*} with $T = T(s_1, \ldots , s_{t-1}, r)$ such that $\sum_{x \in S_1}x = \ldots = \sum_{x \in S_n} x$. As $T(s_1, \ldots , s_{t-1}, r)$ is a function with $t-1$ exponentials, the bound on $|S_i|$ depends by a function $t$ exponentials.

There exist subsets $\bar{C}_1 \subseteq C_1, \ldots , \bar{C}_n \subseteq C_n$ with $p(\bar{C}_1) = S_1, \ldots , p(\bar{C}_n) = S_n$. Hence, we can define the solution $\bar{y} \leq y$ by $\bar{y}^{(i)} = \sum_{c \in \bar{C}_i} \bar{p}(c)$ for every $i>0$, where $\bar{p}$ is the function that projects a vector to the entries that belong the matrix $B^{(i)}$ i.e. $\bar{p}(c) = \bar{p}(\begin{pmatrix} c^{(0)} \\ c^{(i)} \end{pmatrix}) = c^{(i)}$. For $i=0$ we define $y^{(0)} = \sum_{c \in \bar{C}_i} p(c)$. As the sum $\sum_{c \in \bar{C}_i} p(c)$ is identical for every $1 \leq i \leq n$, the vector $\bar{y}$ is a well defined.
\end{proof}



Let $\mathcal{A}$ be a submatrix of $\mathcal{M}$ which corresponds to a subtree with the root matrix $A$. Let $B^{(1)}, \ldots , B^{(n)}$ be the matrices corresponding to the subtrees auf $A$. 

Our goal is to compute for every right hand side vector $b$ with $b = \mathcal{A} y$ for some $y$ with $\norinf{y} \leq T$ the vector $y^*$ with optimal objective. The following algorithm computes those optimal solutions for each right hand side bottom up.
\begin{itemize}
    \item Given right hand side vector $b$.
    Compute for every $y^{(0)}$ with $\norinf{y^{(0)}} \leq T$ the objective value of the solution $y$ consisting of $y^{(0)}$ and the vectors $y^{(1)}, \ldots , y^{(n)}$. Thereby $y^{(i)}$ is the optimal solution of the submatrix $B$ with right hand side $\bar{A}^{(i)} y^{(0)}$, i.e. 
    \begin{align*}
        B^{(i)} y^{(i)} = b- \bar{A}^{(i)} y^{(0)}\\
        \bar{\ell}^{(i)} \leq y^{(i)} \leq u^{(i)}
    \end{align*}, where $\bar{A}^{(i)}$ is the submatrix of $A$ consisting only of rows that belong to $B^{(i)}$ and . By this we ensure that $\mathcal{A}y = b$.
    
    In the case that the matrix $\mathcal{A}$ corresponds to a leave in the tree, there is no submatrix $B^{(i)}$ and we can compute an optimal solution directly by using \cite{eisenbrand2018proximity}.
    
    \item Choose a vector $y$ with optimal objective for each right hand side $b$.
\end{itemize}
Starting at the leaves, we can compute the solutions for each submatrix $\mathcal{A}$ and each right hand side $b$ bottom up.




\begin{proof}
First, we describe the multisets $T_1, \ldots, T_n \subset \ZZgeq^d$ by vectors $\lambda^{(1)}, \ldots , \lambda^{(n)} \in \ZZgeq^{P}$, where $P \subset \ZZ^d$ is the set of integer points $p$ with $\norinf{p} \leq \Delta$. Each $\lambda^{(i)}_{p}$ thereby states the multiplicity of vector $p$ in $T_i$. Hence $\sum_{t \in T_i} t = \sum_{p \in P} \lambda^{(i)}_{p} p$ and our objective is to find vectors $\gamma^{(1)}, \ldots, \gamma^{(n)}$ with $\gamma^{(i)} \leq \lambda^{(i)}$ such that $\sum_{p \in P} \gamma^{(1)}_{p} p = \ldots = \sum_{p \in P} \gamma^{(n)}_{p} p$.

Consider the linear program 
\begin{align*}
    \{ x \in \RRgeq^P \mid \sum_{p \in P} x_p p = b\}.
\end{align*} 
Let $x^{(1)}, \ldots , x^{(\ell)}$ be all possible basic feasible solutions of the LP corresponding to bases $B^{(1)}, \ldots , B^{(\ell)} \in \ZZgeq^{d \times d}$ i.e. $B^{(i)} x^{(i)} = b$.




Clearly, each representation $\lambda^{(i)}$ is also a solution of the linear program. By standard LP theory, we know that each solution of the LP is a convex combination of the basic feasible solutions $x^{(1)}, \ldots , x^{(\ell)}$. Hence, each representation $\lambda^{(i)}$ can be written as a convex combination of $x^{(1)}, \ldots , x^{(\ell)}$, i.e. for each $\lambda^{(i)}$, there exists a $t \in \RRgeq^\ell$ with $\norone{t} = 1$ such that $\lambda^{(i)} = \sum_{i=1}^\ell t_i \bar{x}^{(i)}$, where $\bar{x}^{(i)}_p = \begin{cases} x^{(i)}_p &\text{ if } p \in B^{(i)} \\ 0 & \text{ otherwise}\end{cases}$. By the pigeonhole principle, there exists for each representation $\lambda^{(i)}$ an index $j$ with $t_j \geq  \frac{1}{\ell}$. In the following we will prove that there exists a common point $q \in \ZZgeq^d$ such that for every $x^{(j)}$ there is a $\gamma^{(j)} \in \ZZgeq^d$ with $q = B^{(j)} \gamma^{(j)}$ and $\gamma^{(j)} \leq \frac{1}{\ell} x^{(j)}$.

%This implies that  hence $\gamma^j \leq \lambda^i$.

By Lemma \ref{lem:intersection_all} there exists a set of generating elements $\hat{B}$ such that 
\begin{itemize}
    \item $int.cone(\hat{B}) = \bigcap_{i=1}^n int.cone(B^{(i)})$ and $int.cone(\hat{B}) \neq \{ 0 \}$ as $b \in cone(\hat{B})$ and
    \item each generating vector $\hat{v} \in \hat{B}$ can be represented by $\hat{v} = B^{(i)} x$ for some $x \in \ZZgeq^d$ with $\norone{x} \leq O((d \Delta)^{d (\ell-1)})$ for each basis $B^{(i)}$.
\end{itemize}
Since $b \in cone(\hat{B})$ the vector $\frac{1}{\ell} b$ is also in the cone, i.e. $\frac{1}{\ell} b \in cone(\hat{B})$. Hence, there exists a vector $\hat{\lambda} \in \RRgeq^{\hat{\BB}}$ with $\hat{\BB} \hat{\lambda} = \frac{1}{\ell} b$. Now assume that $\hat{\lambda}_q \geq 1$ for some $q \in \hat{\BB}$. Then $\frac{1}{\ell} b$ can be written by $\frac{1}{\ell} b = q + q'$ for some $q' \in cone(\hat{B})$. As $q$ and $q'$ are contained in the intersection of all cones, there exists for each generating set $\BB^{(j)}$ vectors $\gamma^{(j)} \in \ZZgeq^{\BB^j}$ and $\delta^{(j)} \in \RRgeq^{\BB^{(j)}}$ such that $\BB^{(j)} \gamma^{(j)} =q$ and $\BB^{(j)} \delta^{(j)} = q'$. Hence $\frac{1}{\ell} x^{(j)} = \gamma^{(j)} + \delta^{(j)}$ and we finally obtain that $\frac{1}{\ell} x^{(j)} \geq \gamma^{(j)}$ for $\gamma^{(j)} \in \ZZgeq^{\BB^{(j)}}$.

To prove the existence of the $\gamma^{(j)}$ with $B^{(j)} \gamma^{(j)} = q$ for every $\lambda^{(i)}$ such that $\gamma^{(j)} \leq \lambda^{(i)}$, it only remains to prove the following claim. Note that we choose the weights in $\gamma^{(j)}$ only from a set of $d$ different points in $P$. We write $\gamma^{(j)} \leq \lambda^{(i)}$ in the sense that $\gamma^{(j)}_p \leq \lambda^{(i)}_p$ for each $p \in B^{(j)}$.

\textbf{Claim:} If there is a $\lambda^{(i)}$ with $\norone{\lambda^{(i)}} > d^2 \Delta \ell \cdot O((d \Delta)^{d(\ell-1)})$ then there exists a vector $\hat{x} \in \RRgeq^{\hat{B}}$ with $\hat{\BB} \hat{\lambda} = \frac{1}{\ell}b$ and a point $q \in \hat{B}$ such that $\hat{\lambda}_q \geq 1$.


%It remains to prove that if $\norone{\lambda^i}$ is sufficiently large for $1 \leq i \leq n$, i.e. $\norone{\lambda^i} > d^2 \Delta \ell \cdot O((d \Delta)^{d(\ell-1)})$ then there exists a vector $\hat{x} \in \RRgeq^{\hat{B}}$ with $\hat{\BB} \hat{\lambda} = \frac{1}{\ell}b$ and a point $p \in \hat{B}$ such that $\hat{\lambda}_p \geq 1$. 

To prove the claim, we show that $\norone{\lambda^{(i)}} \leq d \Delta \ell \cdot O((d \Delta)^{d(\ell-1)}) \norone{\hat{\lambda}}$. By Caratheodory \cite{schrijver1998theory} we can then assume that the number of non-zero components of $\hat{\lambda}$ is less or equal than $d$. Hence if $\norone{\lambda^{(i)}} > d^2 \Delta \ell \cdot O((d \Delta)^{d(\ell-1)})$, we know by the pigeonhole principle that there has to exist a point $q \in \hat{B}$ with $\hat{\lambda}_q \geq 1$.

As $\sum_{p \in P} \lambda^{(i)}_p p = b = \sum_{p \in \BB^{(j)}}x^{(j)}_p p$ and every $p \in P$ is bounded by $\norinf{p} \leq \Delta$ we know that \begin{align} 
    \norone{\lambda^{(i)}} \leq d \Delta \norone{x^{(j)}} \label{eq:1}
\end{align} for every $i \leq n$ and every $j \leq \ell$.
Now recall that $\hat{B} \hat{\lambda} = \frac{1}{\ell}b$. By Lemma \ref{lem:intersection_all} we know for each $j \leq \ell$ that 
\begin{align} 
    \norone{x^{(j)}} \leq \ell \cdot O((d \Delta)^{d(\ell-1)}) \label{eq:2} \norone{\hat{\lambda}}
\end{align} as each $v \in \hat{\BB}$ can be written by $\BB^{(i)} \lambda = v$ for some $\lambda \in \ZZgeq^{\BB^{(i)}}$ with $\norone{\lambda} \leq O((d \Delta)^{d(\ell-1)})$. Hence by inequalities \ref{eq:1} and \ref{eq:2} we can conclude that
\begin{align*}
    \norone{\lambda^{(i)}} \leq d \Delta \ell \cdot O((d \Delta)^{d(\ell-1)}) \norone{\hat{\lambda}}
\end{align*}

%Since $\frac{1}{\ell} b \in cone(\hat{B})$, by Caratheodory we can assume that the number of non-zero components of $\hat{x}$ is less or equal than $d$.  and a subset $B^\prime \subseteq \hat{B}$ with $\frac{1}{\ell} b = B'_i x'$. %and the vectors $B^{\prime}_1, \ldots , B^{\prime}_d$ are indecomposable.
%By Lemma \ref{lem:intersection_all}, we know that $\norone{x'} \leq \ell \cdot \Delta^{O(d^{\lceil \log(\ell) \rceil +1})} \norone{x^i}$ for each $1 \leq i \leq \ell$ as each $v \in B'$ can represented by vectors in $B^i$, i.e. $B^i x = v$ for some $\norone{x} \leq \Delta^{O(d^{\lceil \log(\ell) \rceil +1})}$ (note that $v$ is indecomposable). Assuming that $\norone{x^i} \geq d \cdot \ell \cdot (\Delta)^{O(d^{\lceil \log(\ell) \rceil +1})}$, by the pigeonhole principle there exists a coefficient $j$ with $x'_{j} \geq 1$. 




%We define $p$ to be the generating vector corresponding to this specific index, i.e. $p = B'_{j}$ and let $p' = \frac{1}{\ell} b - p$. Clearly, as $p$ and $p'$ are in the intersection of all cones, hence we have that $p \in int.cone(B^i)$ and $p' \in Cone(B^i)$ for all $1 \leq i \leq \ell$.


%\textbf{Claim}: For each $1 \leq i \leq \ell$, there exists a $\gamma^{(i)} \leq \frac{1}{\ell} x^i$ such that $p = B^i \gamma^{(i)}$ \\
%By definition, the vector $\frac{1}{\ell} b$ can be written by the sum of $p$ and $p'$, i.e. $p + p' = \frac{1}{\ell} b$. Since $p,p',(\frac{1}{\ell} b) \in Cone(B^i)$ this implies that $p = B^i \gamma^{(i)} = B^i (\frac{1}{\ell} x^i) - B^i \alpha$ for some $\alpha \in \RRgeq^d$ in the positive orthant with $p' = B^i \alpha$. Hence, $\gamma^{(i)} = \frac{1}{\ell} x^i - \alpha \leq \frac{1}{\ell} x^i$, which proves the claim.

This concludes the proof of Lemma \ref{lem:subrepresentation} as for each representation $\lambda^{(i)}$, we find a basic feasible solution $x^{(j)}$ such that $\frac{1}{\ell}x^{(j)} \leq \lambda^{(i)}$ and further there exists a $\gamma^{(j)} \leq \frac{1}{\ell}x^{(j)}$ with $q = B^{(j)} \gamma^{(j)}$. The size of each $\gamma^{(j)}$ is bounded by $\norone{\gamma^{(j)}} \leq d^2 \Delta \ell \cdot  O((d \Delta)^{d (\ell-1)})$. As $\ell$ is bounded by $\binom{|P|}{d} \leq |P|^d$ and $|P| \leq \Delta^d$, we obtain that \begin{align*}
    \norone{\gamma^{(j)}} \leq d^2 \Delta \ell \cdot O((d \Delta)^{d (\ell-1)}) = (d \Delta)^{O(d (\Delta^{d^2}))}.
\end{align*}
\end{proof}
